Federated Learning Using Variance Reduced Stochastic Gradient for Probabilistically Activated Agents

This paper proposes an algorithm for Federated Learning (FL) with a two-layer structure that achieves both variance reduction and a faster convergence rate to an optimal solution in the setting where each agent has an arbitrary probability of selection in each iteration. In distributed machine learning, when privacy matters, FL is a functional tool. Placing FL in an environment where it has some irregular connections of agents (devices), reaching a trained model in both an economical and quick way can be a demanding job. The first layer of our algorithm corresponds to the model parameter propagation across agents done by the server. In the second layer, each agent does its local update with a stochastic and variance-reduced technique called Stochastic Variance Reduced Gradient (SVRG). We leverage the concept of variance reduction from stochastic optimization when the agents want to do their local update step to reduce the variance caused by stochastic gradient descent (SGD). We provide a convergence bound for our algorithm which improves the rate from $O(\frac{1}{\sqrt{K}})$ to $O(\frac{1}{K})$ by using a constant step-size. We demonstrate the performance of our algorithm using numerical examples.

==> intro_archive.tex <==
\begin{comment}
%In recent years there have been numerous works to design some randomized algorithms to improve the convergence rate of SGD method. 
SGD enjoys cheap iteration cost; however, it suffers from a slow convergence rate because of a decaying step-size and variance that generates due to randomized search. On the other hand, gradient descent (GD) has a fast convergence rate by comparison with SGD. Thus, it is proposed to combine GD with SGD to improve convergence rate of SGD. Many of these methods generally belong to two subclasses. The first one is primal methods of the stochastic gradient descent with variance reduction technique, and the second one is dual methods of the randomized coordinate descent technique. Here for the space limit we just focus on the first class of randomized algorithms. 

\textbf{Stochastic Average Gradient:} The first work done in this class is the Stochastic Average Gradient (SAG)\cite{NLR-MS-FB:12,MS-NLR-FB:17}. The main point in the SAG algorithm is that it stores the average on $m$ gradients of functions $f_i$ evaluated at different points in the memory. Furthermore, the substituted gradient in SAG is not unbiased. As a result, both its biased gradient estimate and bottleneck of memory requirement preclude us to use it even in a small neural network. Afterward, a continued work named SAGA done by \cite{AD-FB:14} alters the SAG algorithm in a way that its substituted gradient becomes unbiased. However, it has memory requirements but it reaches a tighter convergence guarantee compared to SAG.

\textbf{Stochastic Variance Reduced Gradient:} Another variant from the SGD type of methods is Stochastic Variance Reduced Gradient (SVRG). The SVRG algorithm follows two steps with two nested loops. The first step inside the first loop is to compute the full gradient of the function which has an expensive cost, and we try to do it rarely. Sometimes people call this point a snapshot when they want to compute the full gradient of the function, so we refer to this point as a snapshot. The second step inside the second loop is to update the server parameter like the SGD update step but with the substituted gradient term. In other words, the SVRG update looks like the below: 
\begin{align*}
    w &= w - \delta(\nabla f\#(w) -\nabla f\#(w^k) + \nabla f(w^k))
    \\ \text{Where} \quad&\# \quad\text{is chosen randomly}
\end{align*}
Notice that inside the substituted gradient term in SVRG, we compute the stochastic gradient between points $w^k$ and $w$ not the full gradient of the function. The SVRG has more advantages over SAG and SAGA because it does not have memory requirements. However, it needs to compute the full gradient at some snapshots. Furthermore, SVRG works better than SGD as the number of iterations increases because the variance of the iterates is much less than SGD so it directly affects the convergence rate\cite{RJ-TZ:13,JK-PR:17}. Moreover, there has been some work \cite{HW-AB:14} to combine the SVRG with randomized coordinate descent; however, these algorithms need more work to be practical.

 
  



In this era, modern mobile devices have access to plenty of data and most of this data is privacy sensitive. As a result, we cannot train the model by going through the data center. One of the well-known approaches to tackle this problem is using Federated Learning (FL) framework. In FL, we have a server and plenty of devices. Each device owns its private data and then each device does its locally-computed updates via stochastic gradient descent (SGD) on the server parameter. In the end, each device sends its locally updated server parameter. Afterward, by using a simple averaging procedure, as it is done in \cite{HBM-EM-DR-SH-BAA:17}, the server parameter gets updated. This process goes back and forth between the server and devices till the process reaches the optimal model parameter. One of the most practical advantages of FL is that it preserves privacy because of the fact that each agent does its update steps locally and does not share its local data with the other agents. A schematic of FL is shown in Fig \ref{fig:schematic}, where each device has an arbitrary probability of selection. The solution to this problem is of interest in numerous applications such as language models, and image models. Our aim in this paper is to derive a convergence bound and design an algorithm to improve the convergence rate of the proposed algorithm in \cite{JP-SW-MJ-KSC:22} and also reduce the variance produced by SGD update for each agent where each agent has an arbitrary probability of agent selection in each round.





\emph{Literature review}: 
Nowadays, Federated Learning (FL) due to its privacy-preserving property which has been mentioned in \cite{VM-RMP-SP-YH-AD-GS:21,RCG-TK-MN:17,ST-NB-AA-TS-HL-RZ-YZ:19}, and also, training a model in a distributed manner by propagating data across the agents it has received wide interest. However, the original FL algorithm originated from \cite{HBM-EM-DR-SH-BAA:17} where in\cite{XL-KH-WY-SW-ZZ:19,AM-RJ-GJP-HH:21,TL-AKS-MZ-MS-AT-VS:20,SW-TT-TS-KKL-CM-TH-KC:19} they characterize the convergence of FedAvg from a theoretical point of view. Unfortunately, because of the diverseness which exists in the data and system implementing FL in real world problems can be a challenging task. Thus, some works have been done to solve this problem via device scheduling \cite{HHY-ZL-TQQ-HVP:19,YJC-JW-GJ:20,YR-XZ-SCL-CJW:21,HY-MF-JL:21,MC-ZY-WS-CY-HVP-SC:21}. However, in all of these algorithms in this setting, they have used SGD when the agents want to do their update steps. From a stochastic optimization point of view, SGD suffers from both a slow convergence rate because of using a decaying step-size inside the algorithm and high variance which is because of the randomized search of the algorithm. The model proposed in \cite{JP-SW-MJ-KSC:22} is the one most closely related to our work because first, we need to know how our algorithm works in this framework where agents have a non-uniform probability of selection in each round as opposed to the original FedAvg in \cite{HBM-EM-DR-SH-BAA:17} which they uniformly sample agents in each iteration. We will see in the proof and also the simulation part that our algorithm reaches a faster convergence rate and less variance, and it is applicable to be applied to the other algorithms in this setting.

\\





In recent years there have been numerous works to design some randomized algorithms to improve the convergence rate of SGD method. SGD enjoys cheap iteration cost; however, it suffers from a slow convergence rate because of a decaying step-size and variance that generates due to randomized search. On the other hand, gradient descent (GD) has a fast convergence rate by comparison with SGD. Thus, the idea is to combine GD with SGD to compensate for the slow convergence rate of SGD. Many of these methods generally belong to two subclasses. The first one is primal methods of the stochastic gradient descent with variance reduction technique, and the second one is dual methods of the randomized coordinate descent technique. Here for the space limit we just focus on the first class of randomized algorithms. 

\textbf{Stochastic Average Gradient:} The first work done in this class is the Stochastic Average Gradient (SAG)\cite{NLR-MS-FB:12,MS-NLR-FB:17}. The main point in the SAG algorithm is that it stores the average on $m$ gradients of functions $f_i$ evaluated at different points in the memory. Furthermore, the substituted gradient in SAG is not unbiased. As a result, both its biased gradient estimate and bottleneck of memory requirement preclude us to use it even in a small neural network. Afterward, a continued work named SAGA done by \cite{AD-FB:14} alters the SAG algorithm in a way that its substituted gradient becomes unbiased. However, it has memory requirements but it reaches a tighter convergence guarantee compared to SAG.\\
\textbf{Stochastic Variance Reduced Gradient:} Another variant from the SGD type of methods is Stochastic Variance Reduced Gradient (SVRG). The SVRG algorithm follows two steps with two nested loops. The first step inside the first loop is to compute the full gradient of the function which has an expensive cost, and we try to do it rarely. Sometimes people call this point a snapshot when they want to compute the full gradient of the function, so we refer to this point as a snapshot. The second step inside the second loop is to update the server parameter like the SGD update step but with the substituted gradient term. In other words, the SVRG update looks like the below: 
\begin{align*}
    w &= w - \delta(\nabla f\#(w) -\nabla f\#(w^k) + \nabla f(w^k))
    \\ \text{Where} \quad&\# \quad\text{is chosen randomly}
\end{align*}
Notice that inside the substituted gradient term in SVRG, we compute the stochastic gradient between points $w^k$ and $w$ not the full gradient of the function. The SVRG has more advantages over SAG and SAGA because it does not have memory requirements. However, it needs to compute the full gradient at some snapshots. Furthermore, SVRG works better than SGD as the number of iterations increases because the variance of the iterates is much less than SGD so it directly affects the convergence rate\cite{RJ-TZ:13,JK-PR:17}. Moreover, there has been some work \cite{HW-AB:14} to combine the SVRG with randomized coordinate descent; however, these algorithms need more work to be practical.
\\




% \begin{algorithm}[t]
% \begin{algorithmic}[1]
% \caption{FedAvg-SVRG with non-uniformly agent sampling}\label{alg:cap}
% \label{alg:the_alg}
% % \begin{algorithmic}[1]
% \State \textbf{Input:} $\delta$, $K$, $\theta^0$, $\{p_n^k\}$, $S$, $M$
% \State \textbf{Output:} $\theta^k$
% \For{$k \gets 0,..., K - 1$}
%     \State Sample $\vect{1}_n^k \sim p_n^k$
%     \For{$n \gets 1,...,N$}
        
%          \State $ \tilde{w}_{n,0}^k = \theta^k$ 
%          % \State $v_{n}^k=\tilde{w}_n^k$
%          \For{$s \gets 0,...,S-1$}
%          \State $\tilde{w}=\tilde{w}_{n,s}^k$
%             % \State $\tilde{w}_n^k$
%              \State $\tilde{\mu} = \frac{1}{L}\sum_{i=1}^{L} \nabla f_{n,i}(\tilde{w})$\vspace{0.03in}
%              \State $w_{n,0}^k = \tilde{w}$
%              \For{$m \gets 0,...,M-1$}
%                 \State Randomly pick $\# \in \{1,...,L\}$\vspace{0.03in}
%                 \State $w_{n,s,m+1}^k =w_{n,s,m}^k - \delta v_{n,s,m}^{k}$\vspace{0.04in}
%                 \State Where $v_{n,s,m}^{k}= \nabla f_\#(w_{n,s,m}^k)$\vspace{0.04in}
%                \State $- \nabla f_\#(\tilde{w})+\tilde{\mu}$
%                 \EndFor
%             \State \textbf{Option I:} set $\tilde{w}_{n,s+1}^k= w_{n,s,m}^k $ 
%             \vspace{0.01in}
%             \State \textbf{Option II:} set $\tilde{w}_n^k = w_{n,s,m}^k$ \hspace{2cm}\State For randomly chosen $m \in \{0,...,M-2\}$
%         \EndFor
%     \EndFor
%     \State $\theta^{k+1} = \theta^k + \frac{1}{N}\sum_{n=1}^{N} \frac{\vect{1}_n^k}{p_n^k}(w_{n,s,m}^k -\tilde{w}_{n,0}^k )$
%     \EndFor
% \end{algorithmic}
% \end{algorithm}

\emph{Statement of contributions}: 
  In this paper, we propose an algorithm in the FL in the setting where each agent has a non-uniformly probability in each iteration that achieves the following goals: (\emph{i}) The proposed algorithm has a faster convergence rate to the optimal cost in this setting. By theoretical proof, our convergence analysis results in establishing a practical bound for our algorithm which establishes a rate  $O(\frac{1}{K})$ in this setting. (\emph{ii}) We show via the circular error probable (CEP) graph that our algorithm drastically decreases the variance produced by SGD in this framework which results in faster convergence. Hereby, we combine a stochastic optimization technique called SVRG method inside the FL algorithm where each agent has a non-uniformly probability in each round.  
  \end{comment}
  

